Deep RC: A Scalable Data Engineering and Deep Learning Pipeline

Significant obstacles exist in scientific domains including genetics, climate modeling, and astronomy due to the management, preprocess, and training on complicated data for deep learning. Even while several large-scale solutions offer distributed execution environments, open-source alternatives that integrate scalable runtime tools, deep learning and data frameworks on high-performance computing platforms remain crucial for accessibility and flexibility. In this paper, we introduce Deep Radical-Cylon(RC), a heterogeneous runtime system that combines data engineering, deep learning frameworks, and workflow engines across several HPC environments, including cloud and supercomputing infrastructures. Deep RC supports heterogeneous systems with accelerators, allows the usage of communication libraries like MPI, GLOO and NCCL across multi-node setups, and facilitates parallel and distributed deep learning pipelines by utilizing Radical Pilot as a task execution framework. By attaining an end-to-end pipeline including preprocessing, model training, and postprocessing with 11 neural forecasting models (PyTorch) and hydrology models (TensorFlow) under identical resource conditions, the system reduces 3.28 and 75.9 seconds, respectively. The design of Deep RC guarantees the smooth integration of scalable data frameworks, such as Cylon, with deep learning processes, exhibiting strong performance on cloud platforms and scientific HPC systems. By offering a flexible, high-performance solution for resource-intensive applications, this method closes the gap between data preprocessing, model training, and postprocessing.

==> tex/discussion.tex <==
\section{Discussions}
\label{sec:discussions}

Cylon-RP results in \ref{subsec:exp-join},~\ref{subsec:exp-sort} show that Radical-Cylon scales efficiently with very small overheads and outperforms MPI-Cylon in ~\ref{subsec:exp-rp-cylon-mpi-cylon}. In specific, RP-Cylon overheads presented in Table~\ref{tab:a-b-exp_table} show that RP-Cylon takes an average of 3.4 seconds to construct an~\texttt{MPI-Communincator} with 518 ranks which are marginal compared to the total execution time and the size of the experiments.

Cylon performance is measured with a data frame execution runtime. A collection of data frame operators can be arranged in a directed acyclic graph (DAG). Execution of this DAG can further be improved by identifying independent branches of execution and executing such independent tasks parallelly. Additionally, each of these tasks themselves is Bulk Synchronize Parallel (BSP) (this is not the case in most of the engines that are available today). RP-Cylon integration allows us to control the parallelism of these BSP tasks. 
In the future, Cylon is planning to add an optimizer based on the data frame DAG. One aspect is traditional query optimization, similar to SQL query optimization, which is orthogonal to the scheduling mechanism. Another important metric would need would be, what is the scheduling overhead distribution of the underlying scheduling environment.

RP has been meticulously crafted to address a unified execution setting encompassing both CPUs and GPUs, catering to the needs of multiple data pipelines. While integrating CPUs and GPUs within a single task does introduce computational intricacies owing to the foundational structure of Cylon, the concept of heterogeneous execution remains viable. This involves employing distinct groups of ranks equipped with specialized memory allocated either on CPUs or GPUs, enabling the concurrent utilization of these processing units.

The design of RADICAL-Pilot aims to support an extensive spectrum of meticulous resource management policies. Our initial focus has revolved around establishing multiple data pipelines and executing distributed operations in the form of functions. Here Cylon plays an important part by providing distributed execution. Looking ahead to more complex multi-tenancy scenarios, RADICAL-Pilot must proficiently manage a diverse range of resource types, including not only device and host memory but also network bandwidth. The Master-Worker raptor model employed by RADICAL-Pilot provides the system with a robust capability to monitor available resources and allocate them on a large scale. Our future plans involve exploring common multi-tenancy requirements such as prioritization, performance segregation, and resource tracking. Importantly, the timeframe for these endeavors will be considerably shorter than prior efforts yet will encompass significantly larger pools of resources.



==> tex/in2.tex <==
\section{Introduction}\label{sec:introduction}
It is a significantly complex and challenging task to manage and prepare massive data for deep learning in big data science which introduces additional difficulty in model training causing impact on fields such as genomics, climate modeling and astronomy ~\cite{McKenna2010The}.  In addition, data coming from multiple sources often characterized by heterogeneity, high dimensionality, and complex relationships between variables, making it challenging to analyze data using traditional analysis tools. Even with the most advanced computing systems, processing massive datasets can be a significant bottleneck. %Moreover, the sheer volume of data can make storing and transferring data across systems challenging.
While proprietary solutions such as Google Pathways\cite{barham2022pathways, introduc61:online} and OneFlow\cite{yuan2021oneflow} address some aspects of these challenges, there is a critical need for open-source, scalable tools that can be deployed on different cloud and HPC platforms.

While proprietary solutions such as Google Pathways\cite{barham2022pathways, introduc61:online}, OneFlow\cite{yuan2021oneflow}  exist, the need for open-source, scalable runtime tools and data frameworks on HPC platforms is crucial to effectively tackle these challenges. Our goal is to develop a unified approach that combines data engineering and deep learning frameworks with diverse execution capabilities, which can be deployed on various HPC platforms, including cloud systems and supercomputers. 
%Integrating scalable HPC runtime tools with data frameworks is vital for creating scalable solutions for processing large-scale simulations, modeling, and machine learning. 
To address this, Cylon\cite{widanage2020high} offers foundational frameworks for data engineering and deep learning applications on scalable HPC machines. DASK\cite{rocklin2015dask} and SPARK\cite{zaharia2016apache} Dataframe can be alternative to Cylon.  However, Cylon outperforms both in multiple scaling operations\cite{perera2023depth, widanage2020high, abeykoon2020data} although it lacks optimization for efficient resource use and does not support a heterogeneous data pipeline. On the other side, A task-based architecture, RADICAL-Pilot\cite{merzky2022radical} enables Cylon to interact and operate with different HPC platforms seamlessly, shielding Cylon from heterogeneous configurations of different HPC platforms with Radical-Cylon\cite{sarker2024radical} that supports data engineering pipeline. We aim to enhance support for heterogeneous systems with accelerators, enabling frameworks like Cylon with Pytorch and Tensorflow to leverage heterogeneous execution through RADICAL-Pilot and handle data pipeline from data engineering tasks to Deep learning Inferencing jobs. Rapids-cuDF is highly optimized for NVidia GPUs. GPU Cylon is in the pipeline for scaling operations and can be a part of Cylon. RAY\cite{moritz2018ray} provides a distributed runtime that can be an alternative to radical-pilot as a workflow engine. But Ray's GPU support is restricted to scheduling and reservations whereas Radical pilot has the flexibility to control underlying resources. We propose Deep-Cylon, a heterogeneous runtime system with a parallel and distributed data framework designed to execute Cylon tasks within a deep learning pipeline using RADICAL-Pilot. It ensures a complete bridge by creating a data loader with a cylon-distributed data frame that feeds downstream deep learning training and inferencing jobs. Deep-Cylon separates the resource management from the application layer, this would allow Cylon to run on any HPC resources without the need to refactor or rewrite the code, which reduces the development efforts, resulting in a loosely coupled integration. This approach allows the use of heterogeneous communicators across multiple nodes, achieving better performance compared to Bare-Metal Deep Learning execution with minimal overhead. This dual capability promotes collaboration and innovation within the open-source scientific research community.


==> tex/intro.tex <==
\section{Introduction}\label{sec:introduction}

The exponential growth of data volume and complexity creates unprecedented challenges for the scientific community. With the increasing prevalence of sensors, internet-connected devices, and social media, the amount of data being generated is growing at an unprecedented rate. In addition, the complexity of scientific data is also increasing, with data coming from multiple sources often characterized by heterogeneity, high dimensionality, and complex relationships between variables, making it challenging to analyze data using traditional analysis tools. Even with the most advanced computing systems, processing massive datasets can be a significant bottleneck. Moreover, the sheer volume ofx data can make storing and transferring data across systems challenging. 

% and the total computing power in the world has quadrupled due to AI engine deployment


\begin{comment}
High-performance computing clusters have become more important for deep learning model analysis of big data sets. However, this is only one of several difficulties the data processing environment faces. Supporting data engineering for pre-processing, post-processing, communication, and system integration are additional difficulties. To boost user productivity and efficiency, data analytics solutions must be simple to integrate with already-existing frameworks in a variety of languages. This necessitates an effective and widely distributed data processing strategy, but many of the data analytics solutions available today are unable to satisfy all of these demands simultaneously. 
\end{comment}

These challenges have far-reaching implications across various scientific domains, including but not limited to genomics, climate modeling, physics simulations, and neuroscience. In genomics, for example, the amount of data generated from a single genome sequencing has grown exponentially, with individual genome sequencing now generating over 200GB of data~\cite{McKenna2010The}. Processing and analyzing such data using traditional methods can take months or even years. Similar to genomics, a single climate modeling simulation can generate vast amounts of data, with some simulations producing up to 10PB of data. Apart from huge growth, a data science survey conducted by Anaconda, indicates that a considerable amount of developer time (45\%) is dedicated to tasks like data exploration, preprocessing, and prototyping along with 33\% on deep learning tasks \cite{anaconda:online}. 

Analyzing and extracting insights from such massive data sets can be difficult, requiring a paradigm shift in how data analysis is performed, with the need for more efficient and scalable data analysis tools. Finding scalable solutions for processing data, such as large-scale simulations, modeling, and machine learning, is crucial for domain science, as it enables researchers to extract insights and knowledge from vast amounts of data efficiently. These solutions can directly impact reducing the time to solution and cost associated with data analysis by order of magnitudes, allowing scientists to focus on understanding complex systems that are not possible with smaller datasets and conduct more comprehensive and accurate analyses, leading to more robust and reliable results.

\begin{comment}
Modern data engineering frameworks must utilize the full potential of clusters to feed data to applications effectively. However, HPC frameworks like MPI, PGAS, or Slurm are not directly compatible with modern big data systems. Big data frameworks have made an effort to compete by offering comparable APIs, but doing so has a negative impact on performance because it requires switching between runtimes. Thus, there is a critical need for solutions that can leverage the processing power of HPC systems enabling analysis frameworks to accelerate their tasks while efficiently handling large datasets. 

Performing distributed operations quickly leads to faster results from data processing applications. Execution in parallel can improve the performance of aggregation procedures. Aggregations and grouping also need distributed execution to boost scalability given the volume of data created nowadays. Aggregation and grouping procedures are made more complex by parallel and dispersed execution, though. It is difficult but increases AI/ML user productivity to hide these intricacies from AI/ML users and give them access to a simple, recognizable abstraction. 
\end{comment}

Such solutions can be achieved by integrating existing scalable HPC runtime tools with data frameworks. Nevertheless, these solutions impose many research questions, such as performance optimization, programming models, efficient scalability, resource management, and utilization. Cylon\cite{abeykoon2020data} provides underlying frameworks for data engineering and deep learning applications to run on scalable HPC machines. However, it is not optimized for the efficient use of system resources and does not support a heterogeneous data pipeline. 
%To answer these questions, 
So, we first focus on a Python runtime engine that efficiently executes heterogeneous workloads of both executables/Python functions (non)MPI on a set of HPC machines. A task-based architecture, RADICAL-Pilot enable Cylon to interact and operate with different HPC platforms seamlessly, shielding Cylon from heterogeneous configurations of different HPC platforms. RADICAL-Pilot separates the resource management from the application layer, this would allow Cylon to run on any HPC resources without the need to refactor or rewrite the code, which reduces the development efforts, resulting in a loosely coupled integration. 

Furthermore, Cylon requires a heterogeneous runtime environment that constructs a private MPI/UCX/GLOO communicator for every Cylon task on HPC machines, which can be delivered using RADICAL-Pilot. Adding heterogeneous capabilities with RADICAL-Pilot and Cylon framework, which we call Radical-Cylon, can provide a powerful solution to these challenges as it enables the development of a unified system that can handle both compute and data-intensive workloads in an efficient and scalable manner. The experimental outcomes demonstrate that Radical-Cylon performs comparable to Bare-Metal (BM)-Cylon in strong and weak scaling scenarios involving join and sort operations. Radical-Cylon outperforms BM-Cylon in certain instances, particularly when the parallelism level reaches 512 or higher. For heterogeneous execution with strong and weak scaling of multiple tasks (e.g. combination of sort and join), Radical-Cylon showcases a performance improvement of (4$\sim$15)\% faster compared to batch execution with the same amount of resource utilization across all configurations with datasets of 35 million and 3.5 billion rows.

\begin{comment}
\textbf{\textcolor{red}{An unanswered question is what does RADICAL-Cylon enable that was impossible otherwise? The paragraph above seems to imply that the integration leads to a modest quantitative improvement? Are there new capabilities (qualitative) or larger scales that are now feasible that were not earlier?}}

\textbf{\textcolor{blue}{Arup: Cylon uses pre-determine resource allocation with batch execution sequentially to execute multiple tasks. Masters and workers architecture makes it more efficient to schedule task in parallel with allocated resources.}} 
\textbf{\textcolor{red}{Shantenu: What is the measure of "efficiency" ?Can you point me to which figure, please, where we show greater resource utilization or scale?}}

\textbf{\textcolor{blue}{Arup: Please check the \textbf{Benchmarking with multiple data pipeline} graphs. The last 3 graphs. Bar graph presents efficiency in terms of reducing execution time (4-15)\%}} 

\mtnote{While the results show a better efficiency with RP, that might not be related to ``Masters and workers architecture makes it more efficient to schedule task in parallel with allocated resources'' because, as we discussed, it appears that we run only 1 task with RP. Do you confirm that this is indeed the case? If it is, how do you explain the better performance with RP? \\
In Discussion, you write: ``Additionally, each of these tasks themselves is Bulk Synchronize Parallel (BSP). Radical-Cylon integration allows us to control the parallelism of these BSP tasks'' but does the term `task' correspond to a task in RP? Or does it relate to a task within Cylon? If so, RP would not offer any advantage as those `tasks' would be scheduled/managed by Cylon, not RP. If the two tasks are different, then I still do not understand why RP performs better than Cylon when running standalone. On the contrary, if the two task are the same, then I think we should explain that better when describing the experiments and discussing their results.}

\textbf{\textcolor{blue}{Arup: Please check the \textbf{Results shows better when we are running multiple RP tasks(e.g. sort and join)
For BSP, Cylon BSP task is not same as RP task. The Cylon BSP task is divided across multiple parallelisms. RP does not perform better than Cylon on a standalone task. Error bars overlaps each other. We argued results are comparable. It performs better when we perform multiple RP Tasks.}} }

\end{comment}





==> tex/objective.tex <==
\section{Design}
\label{sec:design}

%CYLON and RADICAL-Pilot are two isolated systems offering different functionalities and capabilities. 
The increased features of the proposed design on Cylon include the ability to use GLOO~\cite{gloo:online} and NCCL~\cite{nccl:online} as the communication backend for distributed operations. The design promotes a loosely linked strategy in which both systems take advantage of each other's strengths while operating independently of one another with few dependencies and interactions. In order to exploit the preprocessed Cylon dataframe as input for the Deep Learning system, we offer a distributed data loader for the Cylon data frame. We present two types of bridges: System Bridge, which controls the flow and resources from Cylon to RADICAL-Pilot(RP), and Data Bridge, which links Cylon to the Deep Learning framework. The entire system is referred to as Deep-Cylon.    


In Fig.~\ref{fig:deepcylon-arch}, to submit various Deep-Cylon tasks (services, functions, or executables) to RADICAL-Pilot for multi-node (CPUs and GPUs) execution, Cylon is connected as a top-level client program. It adheres to master-workers designs, in which several worker nodes are under the authority of one or more masters, each of which may have one or more CPUs.  

\begin{figure}[htpb]
    \begin{center}
        \includesvg[width=0.7\linewidth]{Figure/Deep-cylon1.svg}
        \end{center}
        \caption{Deep-Cylon Workflow Architecture. From the bottom-up view, the compute node is a Hardware layer that is compatible with vendor-based CPUs and GPUs. Deep-Cylon tasks consist of data engineering and deep learning jobs executed on multiple execution pipelines.}
    \label{fig:deepcylon-arch}
\end{figure}

%In the initial step (Step 1), when a user intends to
Now let's run a program that uses the Deep-Cylon system to perform several computations by calling the RP-Client(1). Next, the Pilot Manager registers these computations with the Resource Manager and assigns virtual devices for calculations that haven't been run yet (2). The RP-Client then instructs the background server to carry out the pilot manager's instructions, taking into account, among other computations, network connections between devices and data routing activities (3, 4). It is possible to quickly reuse the created representation if the virtual device for a program stays the same. Recompilation is required, nevertheless, if the Resource Manager modifies a program's virtual device. The front end of Deep-Cylon is made up of these three phases together. In order to provide distributed coordination, which makes up the control plane communication, Remote Agent generates numerous execution pipelines with two persistent daemons, an executor and a scheduler, that are capable of communicating (5, 6, 7). In order to build a distributed data loader (8) and carry out local sorting, joining, or deep learning inferencing tasks, the executor calls the Deep-Cylon bridge. In this case, cluster communications involving shuffle, gather, or gradient-sharing activities make up the majority of data plane communications (9). Remarkably, the data plane uses the same communication framework for communication; higher bandwidth is indicated by a blue arrow for the former and lesser bandwidth by a green arrow for the latter.  

Since both systems have straightforward, adaptable Python-based interfaces, their native APIs serve as the primary means of communication between them ~\cite{de_dynamio_2007}. In terms of flexibility, both systems are evolving quickly and may bring about new, significant modifications to the implementation or design, such as the addition or deletion of new system components. Any component that fails can be isolated and contained, keeping the remainder of the system from receiving or performing tasks.

%The main communication point between both systems is their native APIs, as both systems offer flexible and simple Python-based interfaces ~\cite{de_dynamio_2007}. Flexibility-wise, both systems are developing rapidly and might introduce new fundamental changes in the design or implementation, such as adding or removing new system components. 
%Further, any changes in both systems do not necessarily require changes to the other system's components and would not affect the existing integration as there are no direct dependencies between the integrated systems. 
%From a fault tolerance perspective, the integration approach of Cylon and RADICAL-Pilot is more resilient, as failures in one system or component do not affect the entire system. 
%Failure of any component can be isolated and contained, allowing the rest of the system to continue receiving and executing tasks.

